DKMGP: A Gaussian Process Approach to Multi-Task and Multi-Step Vehicle Dynamics Modeling in Autonomous Racing

Autonomous racing is gaining attention for its potential to advance autonomous vehicle technologies. Accurate race car dynamics modeling is essential for capturing and predicting future states like position, orientation, and velocity. However, accurately modeling complex subsystems such as tires and suspension poses significant challenges. In this paper, we introduce the Deep Kernel-based Multi-task Gaussian Process (DKMGP), which leverages the structure of a variational multi-task and multi-step Gaussian process model enhanced with deep kernel learning for vehicle dynamics modeling. Unlike existing single-step methods, DKMGP performs multi-step corrections with an adaptive correction horizon (ACH) algorithm that dynamically adjusts to varying driving conditions. To validate and evaluate the proposed DKMGP method, we compare the model performance with DKL-SKIP and a well-tuned single-track model, using high-speed dynamics data (exceeding 230kmph) collected from a full-scale Indy race car during the Indy Autonomous Challenge held at the Las Vegas Motor Speedway at CES 2024. The results demonstrate that DKMGP achieves upto 99% prediction accuracy compared to one-step DKL-SKIP, while improving real-time computational efficiency by 1752x. Our results show that DKMGP is a scalable and efficient solution for vehicle dynamics modeling making it suitable for high-speed autonomous racing control.

==> modeling.tex <==
%Before formulating the problem that integrates the Extended Kinematic (E-kin) model with the proposed DKMGP model to enhance dynamics modeling accuracy, 
We first present a brief overview of the single-track and the E-kin models used in this paper. 

\begin{table*}[]
    \scriptsize
    \centering
    \caption{E-kin model and single-track model state equations; highlighted states differ between the models, including the Pacejka tire model equations}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l l l}
        \hline
        \textbf{State Variable} & \textbf{Notation} & \textbf{State Equation (E-Kin)} & \textbf{State Equation (Single-track)} \\
         Horizontal Position (\si{\meter}) & $x$ & $\dot x = v_{x}\cos\psi - v_{y}\sin\psi$ & $\dot x = v_{x}\cos\psi - v_{y}\sin\psi$ \\
         Vertical Position (\si{\meter}) & $y$ & $\dot y = v_{x}\sin\psi_t + v_{y}\cos\psi$ & $\dot y = v_{x}\sin\psi + v_{y}\cos\psi$ \\
\rowcolor{lightgray}         
Longitudinal Velocity (\si{\meter\per\second}) & $v_x$ & {$\dot v_{x}$} $= \frac{T_w}{l_r+l_f}a_x$ & {$\dot v_{x}$} $= a_x$ \\[3pt]
\rowcolor{lightgray}           
Lateral Velocity (\si{\meter\per\second}) & $v_y$ & {$\dot v_{y}$} $= \frac{1}{T_w(l_r+l_f)}(a_x\sin\psi+ v_x\omega)$ & {$\dot v_{y}$} $= \frac{1}{m}(F_{ry}+F_{fy}\cos\delta-F_{by})- v_x\omega$ \\
       
Inertial Heading (\si{\radian}) & $\psi$ &  $\dot \psi = \omega$ & $\dot \psi = \omega$ \\[3pt]
         Steering Angle (\si{\radian})& $\delta$ & $\dot \delta = \Delta\delta$ & $\dot \delta = \Delta\delta$ \\
\rowcolor{lightgray}            
 Yaw Rate (\si{\radian\per\second}) & $\omega$ & {$\dot \omega$} $= \frac{h_{cog}}{T_w(l_r+l_f)}(a_x\cos\psi+ v_x\omega)$ & {$\dot \omega$} $= \frac{1}{I_z}(l_{f}F_{fy}\cos\delta-l_{r}F_{ry})$ \\[3pt]
         
        \hline
        \textbf{Tire Forces (Pacejka)} & & & \\
        Front Lateral Tire Force (\si{\newton}) & $F_{yf}$ & \multicolumn{2}{l}{$F_{yf} = Svy_{f} + D_f \sin( C_f \arctan ( B_f \alpha_f - E_f( B_f \alpha_f  -\arctan(B_f \alpha_f))))$} \\[3pt]
        Rear Lateral Tire Force (\si{\newton}) & $F_{yr}$ & \multicolumn{2}{l}{$F_{yr} = Svy_{r} + D_r \sin( C_r \arctan( B_r \alpha_r - E_r( B_r \alpha_r - \arctan(B_r \alpha_r))))$} \\[3pt]
        Front Slip Angle (\si{\radian}) & $\alpha_f$ & \multicolumn{2}{l}{$\alpha_f = \alpha_{f0} + Shy_{f}, \quad \alpha_{f0} = \delta - \arctan \left(\frac{v_y + l_f \omega}{v_x}\right)$} \\[3pt]
        Rear Slip Angle (\si{\radian}) & $\alpha_r$ & \multicolumn{2}{l}{$\alpha_r = \alpha_{r0} + Shy_{r}, \quad \alpha_{r0} = -\arctan \left(\frac{v_y - l_r \omega}{v_x}\right)$} \\
        \hline
    \end{tabular}
    }
    \label{tab:dynamics_equations}
\end{table*}
\vspace{-5pt}
\subsection{Single-track Model}
The single-track model, as shown in Fig.\ref{fig:single-track}, simplifies the vehicle dynamics by combining the two wheels of both the front and rear axles into a single wheel per axle. This model is commonly used for motion planning and real-time vehicle control (\cite{raji2022motion, liniger2015optimization}.) The differential equations of state descriptions of the single-track model are shown in the Table~\ref{tab:dynamics_equations}, where the vehicle state is composed of $s=\{x, y, v_x, v_y, \psi,$ $\delta, \omega\}$, and the inputs are $u=\{a_x, \Delta\delta\}$, where $\Delta\delta$ represents the steering velocity, $a_x$ is the longitudinal vehicle acceleration, respectively.
%Specifically, the single-track model used in this paper assumes that 
% The longitudinal dynamics of the racecar are characterized directly by the vehicle's longitudinal acceleration, $a_x$. 
Note that in this work, we simplify the longitudinal dynamics by directly using the vehicle's longitudinal acceleration, whereas in real-world applications, a well-calibrated drivetrain model is necessary to precisely compute the force transferred from the engine to the driving wheels.
The lateral dynamics of the racecar are characterized by states including lateral velocity ($v_y$), yaw rate ($\psi$), steering angle ($\delta$), and yaw rate ($\omega$). 
The associated differential equations incorporate forces such as the lateral tire forces of the front ($F_{fy}$) and rear ($F_{ry}$) axles, and the force due to bank angle ($F_{b_y}$), where $F_{b_y} = mg \sin(\theta)$ approximates the influence of the bank angle $\theta$. Tire forces, $F_{fy}$ and $F_{ry}$, are modeled using the Pacejka magic formula for the tire model, detailed in the bottom of Table~\ref{tab:dynamics_equations}. 
%approximates tire-road interactions using the parameters $B_i$, $C_i$, $D_i$, $E_i$, $Svy_i$, $Shy_i$, which define the shape of the tire force curve in relation to the slip angles $\alpha_i$, where $i$ represents either the front or rear tires. 


\subsection{Extended Kinematic Model}
\setlength{\intextsep}{3pt} % Reduce vertical space above and below
\setlength{\columnsep}{8pt} % Reduce horizontal space to the text
\begin{wrapfigure}{r}{0.4\textwidth}
    \centering
    \includegraphics[width=0.4\textwidth]{images/single-track.pdf}
    \caption{The single-track vehicle model of the racecar, with all three base states $(v_x. v_y, \omega)$ highlighted.}
\vspace{-2pt}
    \label{fig:single-track}
\end{wrapfigure}
Table~\ref{tab:dynamics_equations} demonstrates that all vehicle states can be derived from the base states \( \{v_x, v_y, \omega\} \). While the single-track model simplifies vehicle dynamics modeling, it still requires extensive expert knowledge and calibration. For example, deriving \( \dot{v}_y \) involves lateral dynamics with factors such as aerodynamics and tire forces, while \( \dot{v}_x \) requires understanding longitudinal dynamics, including the powertrain system.
To reduce model development costs, we propose an extended kinematic single-track (E-kin) model, shown in column 3 of Table~\ref{tab:dynamics_equations}. Unlike the nonlinear single-track model, which relies on detailed subsystem modeling, the E-kin model approximates the derivatives of the base states using measurable variables such as \( a_x \), \( \psi \), and \( \delta \). This approach avoids explicit modeling of complex subsystems like tire dynamics and drivetrain dynamics, greatly simplifying and reducing modeling costs.
However, the E-kin model’s simplifications introduce discrepancies between its predictions and real-world vehicle dynamics. Thus, a method is needed to learn and compensate for these mismatches while retaining the model’s simplified calibration benefits.

\subsection{Problem Formulation}
\label{sec:ms}
% To measure the discrepancies between the E-kin model and the actual racecar dynamics, 
Given a dataset \( D =\{d_1, d_2, \dots, d_N\}\) consisting of $N$ vehicle state measurement samples \( S = \{s_1, s_2, \dots, s_N\} \) and inputs \( U = \{u_1, u_2, \dots, u_N\} \), \hl{the objective is to predict future states $\hat{\mathbf{s}}_{t+1}, \hat{\mathbf{s}}_{t+2}, \ldots, \hat{\mathbf{s}}_{t+n}$ using a learned model that corrects for the inherent inaccuracies in the baseline E-kin model.}
At each timestep \( t \), the model predictions, denoted as \( f_{\text{E-kin}}(s_t, u_t) \), are generated by propagating the E-kin model with the same inputs \( u_t =  \{a_{x,t}, \Delta\delta_t\} \) and initial states \( s_t = \{x_t, y_t, v_{x,t}, v_{y,t}, \psi_t, \delta_t, \omega_t\} \). 
Our goal is to correct the \( f_{\text{E-kin}}(s_t, u_t) \) by learning the model mismatch between predictions and ground truth, which is defined as $r_{t+1} = s_{t+1} - f_{Ekin}(s_{t}, u_{t})$. 
% The model's predictions are denoted by \( f_{\text{E-kin}}(s_t, u_t) \) and the residual at time \( t \) is defined as $r_t = s_{t} - f_{Ekin}(s_{t-1}, u_{t-1})$.
% in Equation~\ref{eq:res}. 
The mismatch between the E-kin model and the actual vehicle dynamics is influenced by the base states \( \{v_x, v_y, \omega\} \). 
Therefore, the set of model residuals is defined as \( \mathcal{R} := \{r_1, \ldots, r_{N}\} \), each residual at time \( t \) is given by \( r_t = [0, 0, \epsilon_{v_{x,t}}, \epsilon_{{v_y,t}}, 0, 0, \epsilon_{\omega,t}] \). Here, \( \epsilon_{v_{x,t}}, \epsilon_{{v_y,t}}, \) and \( \epsilon_{\omega,t} \) represent the residuals corresponding to the base states \( \{v_x, v_y, \omega\} \) at time \( t \).
% \begin{equation}
%     r_t = s_{t} - f_{Ekin}(s_{t-1}, u_{t-1})
% \label{eq:res}
% \end{equation}
% We use GP for model residual learning, as 

\noindent\textbf{Problem 1: Multi-task Gaussian Process} 
We use GP model for learning dynamics model mismatches, denoted as $\mathcal{GP}(d_{t-1}) = r_t + \nu_t \approx e_t$. Here, $e_t=\{\epsilon_{{v_x}_t}, \epsilon_{{v_y}_t}, \epsilon_{{\omega}_t}\}$ represents GP estimated model error at time \( t \), and $\nu_t \sim \mathcal{N}(0,1) $ is the additive Gaussian noise. Therefore, we can formulate the corrected model predictions, $f_{corr}$, by combining GP learned model error and E-kin model predictions, $f_{Ekin}$, as shown in Equation \ref{eq:fcorr}.
\vspace{-5pt}
\begin{equation}
    f_{corr}(s_t,u_t) = f_{Ekin}(s_{t-1},u_{t-1}) + e_t \approx s_{t}
\label{eq:fcorr}
\end{equation}
However, existing GP-based methods, such as DKL-SKIP, often require training separate GP models for learning each model error, resulting in high computational costs due to the space and time complexity of GP models. In this paper, we propose a multi-task Gaussian Process (MTGP) framework that predicts all model errors simultaneously, addressing these inefficiencies by reducing the number of required models and leveraging shared information across tasks.

% \vspace{-5pt}
% \vspace{-2pt}
% \begin{equation}
%     \mathcal{GP}(d_{t-1}) = r_t + \nu_t \approx e_t
% \label{eq:GPerr}
% \end{equation}
% \vspace{-5pt}
\noindent\textbf{Problem 2: Multi-step prediction}
% \hl{Despite the DKMGP model improves prediction accuracy and efficiency compared to existing methods, the inherent computational cost of GP model still presents challenges for real-time applications.} 
% \hl{To address this limitation and enable the DKMGP to be suitable for real-time control, such as receding horizon control}, 
We propose a multi-step prediction algorithm, in which, at each time step \(t\), the E-kin model propagates for \(n\) steps using initial states and control inputs, as shown in Equation \ref{eq:ekin_prop}. 
\vspace{-5pt}
\begin{equation}
\begin{array}{ccc}
    \hat{s}_{t+1} = f_{Ekin}(s_t, u_t); & 
    \dots; & 
    \hat{s}_{t+n} = f_{Ekin}(\hat{s}_{t+n-1}, u_{t+n-1}) \\
\end{array}
\label{eq:ekin_prop}
\end{equation}
Then, the model output, $\hat{s}_{t+n}$, is corrected by predictions of the MTGP model, $\mathcal{GP}_n(d_{t}) = r_{t+n} + \nu_{t+n} \approx e_{t+n}$, to approximate the actual dynamics, \(s_{t+n}\), as shown in Equation~\ref{eq:modprop}.
\vspace{-5pt}
\begin{equation}
    f_{corr}(\hat{s}_{t+n},u_{t+n}) = \hat{s}_{t+n} + e_{t+n} \approx s_{t+n} \\
\label{eq:modprop}
\end{equation}


